Sensing-Constrained LQG Control

Linear-Quadratic-Gaussian (LQG) control is concerned with the design of an optimal controller and estimator for linear Gaussian systems with imperfect state information. Standard LQG assumes the set of sensor measurements, to be fed to the estimator, to be given. However, in many problems, arising in networked systems and robotics, one may not be able to use all the available sensors, due to power or payload constraints, or may be interested in using the smallest subset of sensors that guarantees the attainment of a desired control goal. In this paper, we introduce the sensing-constrained LQG control problem, in which one has to jointly design sensing, estimation, and control, under given constraints on the resources spent for sensing. We focus on the realistic case in which the sensing strategy has to be selected among a finite set of possible sensing modalities. While the computation of the optimal sensing strategy is intractable, we present the first scalable algorithm that computes a near-optimal sensing strategy with provable sub-optimality guarantees. To this end, we show that a separation principle holds, which allows the design of sensing, estimation, and control policies in isolation. We conclude the paper by discussing two applications of sensing-constrained LQG control, namely, sensing-constrained formation control and resource-constrained robot navigation.

==> tex/Deprecated_MainResults_Vassilis.tex <==
%!TEX root = ../main.tex

\section{Algorithm for Sensing-Constrained LQG Control}

We present the first scalable algorithm for the sensing-constrained LQG control Problem~\ref{prob:LQG}, and prove that it achieves an approximate value for Problem~\ref{prob:LQG} that is finitely close to the optimal.
To~this~end, we start with the definition of the supermodularity ratio of monotone functions.

\subsection{Supermodularity ratio of monotone functions}

We introduce a definition of supermodularity ratio for monotone functions, which we use in our contributions in this paper.  To this
end, we start with the definitions of non-increasing set functions, and of supermodular set functions.

\begin{mydef}[Monotonicity]
Consider any finite ground set~$\mathcal{V}$.  The set function $f:2^\calV\mapsto \mathbb{R}$ is non-increasing if and only if for any $\mathcal{A}\subseteq \mathcal{A}'\subseteq\calV$, $f(\mathcal{A})\geq f(\mathcal{A}')$. \hfill $\blacktriangle$
\end{mydef}
In words, a set function $f:2^\calV\mapsto \mathbb{R}$ is non-increasing if and only if adding more elements in any $\mathcal{A}\subseteq\mathcal{V}$ cannot increase the value of $f(\mathcal{A})$.
 
\begin{mydef}[Supermodularity (\hspace{-.05mm}\cite{nemhauser78analysis}, Proposition 2.1)]\label{def:sub}
Consider any finite ground set $\calV$.  The set function $f:2^\calV\mapsto \mathbb{R}$ is supermodular if and only if
for any $\mathcal{A}\subseteq \mathcal{A}'\subseteq\calV$ and $x\in \calV$, $f(\mathcal{A})-f(\mathcal{A}\cup \{x\})\geq f(\mathcal{A}')-f(\mathcal{A}'\cup \{x\})$. \hfill $\blacktriangle$
\end{mydef}
In words, a set function $f:2^\calV\mapsto \mathbb{R}$ is supermodular if and only if it satisfies the following intuitive diminishing returns property: for any $x\in \mathcal{V}$, the drop $f(\mathcal{A})-f(\mathcal{A}\cup \{x\})$ diminishes as $\mathcal{A}$ grows; equivalently, for any $\mathcal{A}\subseteq \mathcal{V}$ and $x\in \mathcal{V}$, the drop $f(\mathcal{A})-f(\mathcal{A}\cup \{x\})$ is non-increasing.


\begin{mydef}[Supermodularity ratio]\label{def:super_ratio}
Consider any finite ground set~$\mathcal{V}$, and a non-increasing set \mbox{function $f:2^\calV\mapsto \mathbb{R}$}.  We define the~supermodularity ratio of $f$ as
\begin{equation*}
\gamma_f = \min_{\mathcal{A} \subseteq \mathcal{V}, x, x' \in \mathcal{V}\setminus\calA} \frac{f(\mathcal{A})-f(\mathcal{A}\cup \{x\})}{f(\mathcal{A}\cup\{x'\})-f[(\mathcal{A}\cup\{x'\})\cup \{x\}]}.
\end{equation*}

\vspace{-3mm}
\hfill $\blacktriangle$
\end{mydef}
In words, the supermodularity ratio of a monotone set function $f:2^\calV\mapsto \mathbb{R}$ measures how far $f$ is from being supermodular: in particular, per the Definition~\ref{def:super_ratio} of supermodularity ratio, the supermodularity ratio $\gamma_f$ takes values in $[0,1]$, and
\begin{itemize}
\item $\gamma_f= 1$ if and only if $f$ is supermodular, \mbox{since for $\gamma_f= 1$} Definition~\ref{def:super_ratio} \mbox{implies for any $\calA \subseteq \calV$, and any $x,x' \in \calV$,}
\begin{equation*}
f(\mathcal{A})-f(\mathcal{A}\cup \{x\})\geq f(\mathcal{A}\cup\{x'\})-f[(\mathcal{A}\cup\{x'\})\cup \{x\}],
\end{equation*}
that is, that the drop $f(\mathcal{A})-f(\mathcal{A}\cup \{x\})$ is non-increasing as new elements are added in $\calA$.
\item $0\leq\gamma_f < 1$ if and only if $f$ is approximately supermodular, in the sense that for $\gamma_f< 1$ Definition~\ref{def:super_ratio} implies for any $\calA \subseteq \calV$, and any $x,x' \in \calV$,
\begin{align*}
 f(\mathcal{A})-& f(\mathcal{A}\cup \{x\})\geq \\
&\gamma_f \left\{f(\mathcal{A}\cup\{x'\})-f[(\mathcal{A}\cup\{x'\})\cup \{x\}]\right\},
\end{align*}
that is, that the drop $f(\mathcal{A})-f(\mathcal{A}\cup \{x\})$ is approximately non-increasing as new elements are added in $\calA$; specifically, for any $\calA \subseteq \calV$, and any $x,x' \in \calV$, the supermodularity ratio $\gamma_f$ captures how much ones needs to discount the drop $f(\mathcal{A}\cup\{x'\})-f[(\mathcal{A}\cup\{x'\})\cup \{x\}]$, ---which results from adding the element $x'$ in $\calA$,--- such that the drop $f(\mathcal{A})-f(\mathcal{A}\cup \{x\})$ remains greater then, or equal to, the drop $f(\mathcal{A}\cup\{x'\})-f[(\mathcal{A}\cup\{x'\})\cup \{x\}]$.
\end{itemize}

We next provide an algorithm for the sensing-constrained LQG control Problem~\ref{prob:LQG}; we use the supermodularity ratio Definition~\ref{def:super_ratio} to quantify its approximation performance.

%Several supermodularity ratio definitions have been introduced in the literature of set function optimization~\cite{das2011submodular,wang2016approximation,chamon2016near}; the most relevant to ours ---Definition~\ref{def:super_ratio}--- are the supermodularity ratio definitions in~\cite{wang2016approximation,chamon2016near}.  In~particular, given  a monotone, non-supermodular set function $f:2^\calV\mapsto\mathbb{R}$, in~\cite{wang2016approximation} the notion of elemental curvature $\alpha_f$ is introduced, which is equal to the reciprocal of $\gamma_f$; and in~\cite{chamon2016near}, a notion of supermodular ratio $r_f$ is introduced, which is equal to $\gamma_f^{k_f}$, where $k_f$ is such that $k_f=O(|\calV|)$; that is,  given  a monotone, non-supermodular set function $f:2^\calV\mapsto\mathbb{R}$, $r_f$ is in general smaller that $\gamma_f$, since for a non-supermodular set function $f$, $\gamma_f<1$.
%
%All aforementioned supermodularity ratio introduced  in~\cite{das2011submodular,wang2016approximation,chamon2016near} serve in quantifying the approximation performance of the greedy algorithm to solve the cardinality constraint optimization problem $\min_{\calS \subseteq \calV, |\calS|\leq k}f$, where $f:2^\calV\mapsto\mathbb{R}$ is a monotone set function. 
%In the following paragraphs, we use the notion of supermodularity ration in Definition~\ref{def:super_ratio} to quantify the  the same for the sensing-constrained LQG control Problem~\ref{prob:LQG}.

\subsection{Algorithm for sensing-constrained LQG control}

\begin{mynotation}\label{notation:sensor_noise_matrices}
For any time $t\in \until{T}$, and any sensor set $\calS \subseteq \calV$, let 
\begin{itemize}
\item $C_t(\calS)$ to be the measurement matrix corresponding to the selected sensors in $\calS$, i.e., for $\calS=\{i_1, i_2 \ldots, i_{|\calS|}\}$,
$$C_t(\calS) = [C\at{i_1,t}\tran, C\at{i_2,t}\tran, \ldots, C\at{i_{|\calS|},t}\tran]\tran;$$
\item $V_t(\calS)$ to be the noise covariance matrix corresponding to the selected sensors in $\calS$, i.e., for $\calS=\{i_1, i_2 \ldots, i_{|\calS|}\}$,
$$V_t(\calS)= \text{diag}[V\at{i_1,t}, V\at{i_2,t}, \ldots,V\at{i_{|\calS|},t}];$$
\item for any sensor set $\calS\subseteq\calV$, and any time $t\in \{1,2,\ldots, T\}$, $\hat{x}_{t,\calS}$ to be the Kalman estimator ---minimum mean square estimator--- of the state $x_t$ given the measurements up to time $t$, i.e.~\cite[Appendix~E]{bertsekas2005dynamic},
\begin{equation*}
\hat{x}_{t,\calS}=\mathbb{E}(x_t|y_{1,\calS},y_{2,\calS},\ldots,y_{t,\calS});
\end{equation*}
\item for any sensor set $\calS\subseteq\calV$, and any time $t\in \{1,2,\ldots, T\}$, $\Sigma\att{t}{t}(\calS)$ to be the error covariance of the Kalman estimator $\hat{x}_{t,\calS}$, i.e.~\cite[Appendix~E]{bertsekas2005dynamic},
\begin{equation*}
\Sigma\att{t}{t}(\calS)=\mathbb{E}[(\hat{x}_{t,\calS}-x_t)(\hat{x}_{t,\calS}-x_t)\tran].
\end{equation*}
\end{itemize} 

\vspace{-3mm}
\hfill $\blacktriangle$
\end{mynotation}

\begin{algorithm}[t]
\caption{\mbox{for sensing-constrained LQG control Problem~\ref{prob:LQG}.}}
\begin{algorithmic}[1]
\REQUIRE  Per Problem~\ref{prob:LQG}, the inputs to Algorithm~\ref{alg:greedy} are the:
\begin{itemize}
\item time horizon $T$;
\item available sensor set $\calV$;
\item covariance matrix $\Sigma\att{1}{0}$ of system's initial condition $x_1$;
\item for any time $t \in \{1,2,\ldots, T\}$: system matrix $A_t$; input matrix $B_t$; LQG cost matrices $Q_t$ and $R_t$; and process noise covariance matrix $W_t$; 
\item for any time $t \in \{1,2,\ldots, T\}$, and \mbox{any sensor $i \in \calV$}: measurement matrix $C_{i,t}$; and measurement noise covariance matrix $V_{i,t}$.
\end{itemize}
\ENSURE Sensor set $\widehat{\mathcal{S}}$, and control gain matrices $K_1, K_2$, $\ldots, K_T$, with properties per Theorem~\ref{th:approx_bound}.
\STATE $N_{T+1}\leftarrow 0_{n_{T}\times n_T}$; $t\leftarrow T$;
\WHILE {$t\geq 1$} 
\STATE{$S_t \leftarrow Q_t + N_{t+1}$; $N_t \leftarrow A_t\tran (S_t\inv+B_tR_t\inv B_t\tran)\inv A_t$;}
\STATE{$M_t \leftarrow B_t\tran S_t B_t + R_t$; $K_t \leftarrow - M_t\inv B_t\tran S_t A_t$; $t\leftarrow t-1$;}
\ENDWHILE
\STATE{$t\leftarrow 1$;}
\WHILE {$t\leq T$}
\STATE{$\Theta_t \leftarrow K_t\tran M_t K_t$; $t\leftarrow t-1$;}
\ENDWHILE
\STATE $\mathcal{S}\leftarrow\emptyset$; $i \leftarrow 0$;
\WHILE {$i < k$} 
	\FORALL {$a\in \calV\setminus\widehat{\mathcal{S}}$}
	\STATE{$\widehat{\mathcal{S}}'\leftarrow \widehat{\mathcal{S}}\cup \{a\}$; $\Sigma\att{1}{0}(\widehat{\mathcal{S}}')\leftarrow \Sigma\att{1}{0}$; $t\leftarrow 1$;}
	\WHILE {$t\leq T$}
	\vspace{0.3mm}
	\STATE{$\Sigma\att{t}{t}(\widehat{\mathcal{S}}')\leftarrow$}
	\STATE{$[ 
	\Sigma\att{t}{t-1}(\widehat{\mathcal{S}}')\inv + C_t(\widehat{\mathcal{S}}')\tran V_t(\widehat{\mathcal{S}}')\inv C_t(\widehat{\mathcal{S}}')]\inv$;}
	\STATE{$\Sigma\att{t}{t-1}(\widehat{\mathcal{S}}')\leftarrow A_{t-1} \Sigma\att{t-1}{t-1}(\widehat{\mathcal{S}}') A_{t-1}\tran + W_{t-1}$;}
	\STATE{$t\leftarrow t+1$;}
	\ENDWHILE
	\ENDFOR
\STATE{$a_i \leftarrow a'\in \arg\min_{a \in \calV\setminus \mathcal{S}}\sum_{t=1}^T\text{tr}[\Theta_t\Sigma\att{t}{t}(\widehat{\mathcal{S}}\cup\{a\})]$;}
\STATE{$\widehat{\mathcal{S}}\leftarrow \widehat{\mathcal{S}} \cup \{a_i\}$; $i \leftarrow i+1$;}
\ENDWHILE
\end{algorithmic} \label{alg:greedy}
\end{algorithm}

We provide Algorithm~\ref{alg:greedy} for the polynomial-time solution of the sensing-constrained LQG control  Problem~\ref{prob:LQG}, and characterize its approximation and running time performance.

Algorithm~\ref{alg:greedy} constructs a solution $(\algS, u_{1,\algS}, u_{2,\algS}, \ldots, u_{T,\algS})$ for the sensing-constrained LQG control Problem~\ref{prob:LQG}, where $\algS$ is the sensor set, and $(u_{1,\algS}, u_{2,\algS}, \ldots,u_{T,\algS})$ the control policies,  in two steps:

\textit{a)} \textit{(Controller design)} In lines 1--5, Algorithm~\ref{alg:greedy} constructs the control policies $(u_{1,\algS}, u_{2,\algS}, \ldots,u_{T,\algS})$, by computing the matrices $K_1,K_2,\ldots,K_T$.  In particular, given a sensor set~$\algS$, and measurements $y_{1,\algS},y_{2,\algS},\ldots,y_{t,\algS}$ up to time~$t$,  we prove that the optimal control policy~$u_{t,\algS}$ for the imperfect state information Problem~\ref{prob:LQG} is equal to $K_t\hat{x}_{t,\algS}$.
%; i.e., given a sensor set $\algS$, $K_t$ constructs the control policy $u_{t,\algS}$, and specifically, decides how the Kalman estimate $\hat{x}_{t,\algS}$ of the state $x_t$ affects the control policy~$u_{t,\algS}$.

\begin{myremark}[Certainty equivalence principle]\label{rem:certainty}
In this paper, we prove that the certainty equivalence principle holds for the sensing-constrained LQG control Problem~\ref{prob:LQG}.  In particular, we prove that the control gain matrices $K_1, K_2, \ldots, K_T$, 
which are computed in Algorithm~\ref{alg:greedy}'s lines 1--5,
% and which for any sensor set $\calS \subseteq \calV$ make the control policies $(K_1\hat{x}_{1,\calS}$, $K_2\hat{x}_{2,\calS},  \ldots, K_T\hat{x}_{T,\calS})$ optimal for Problem~\ref{prob:LQG}, 
are the same control gain matrices that make the control policies $(K_1x_1$, $K_1x_2,\ldots, K_T x_T)$ optimal for the perfect state information version of Problem~\ref{prob:LQG}, where at any time $t \in \until{T}$ the state $x_t$ is known~\cite[Chapter~4]{bertsekas2005dynamic}.  \hfill $\blacktriangle$
\end{myremark}

\textit{b)} \textit{(Sensor selection)} In lines 6--23, Algorithm~\ref{alg:greedy} selects greedily a sensor set~$\algS$, among all sensor sets $\calS\subseteq \calV$, to solve Problem~\ref{prob:LQG}, by considering how at any time $t \in \until{T}$ the Kalman estimation error $x_t-\hat{x}_{t,\calS}$ 
%of the Kalman estimate $\hat{x}_{t,\calS}$ of $x_t$
%, i.e., the error between the Kalman estimate $\hat{x}_{t,\calS}$ of the state $x_t$ and the state $x_t$, 
perturbs the control policy $u_{t,\calS}=K_t\hat{x}_{t,\calS}$
%, which given a sensor set $\calS$ we prove to be optimal for Problem~\ref{prob:LQG},
away from the  control policy $K_tx_t$, which is optimal 
for the perfect state information version of Problem~\ref{prob:LQG}.
%, where at any time $t \in \until{T}$ the state $x_t$ is known~\cite[Chapter~4]{bertsekas2005dynamic}.  
In~particular, \mbox{in~lines 6--23}, Algorithm~\ref{alg:greedy} selects greedily a sensor set~$\algS$, among all sensor sets $\calS\subseteq \calV$, to minimize the set function $\sum_{t=1}^{T}\text{tr}[\Theta_t\Sigma\att{t}{t}(\calS)]$, where at any time $t \in \until{T}$, the term $\text{tr}[\Theta_t\Sigma\att{t}{t}(\calS)]$ captures the mean square estimation error that disturbs the control policy $u_{t,\calS}=K_t\hat{x}_{t,\calS}$ away from the perfect state information control policy~$K_tx_t$; the reason for the latter is twofold:
\begin{itemize}
\item for any time $t \in \until{T}$, the matrix $\Theta_t$
%, computed in Algorithm~\ref{alg:greedy}'s lines 6--9, 
incorporates how the Kalman estimation error $x_t-\hat{x}_{t,\calS}$ perturbs the control policy $u_{t,\calS}=K_t\hat{x}_{t,\calS}$ away from the perfect state information control policy $K_tx_t$, since (i)~$u_{t,\calS}=K_t\hat{x}_{t,\calS}=K_tx_t-K_t(x_t-\hat{x}_{t,\calS})$; and (ii)~the matrices $\Theta_t$ and $K_t$ have the same null space, since $\Theta_t= K_t\tran M_t K_t$ per Algorithm~\ref{alg:greedy}'s line~8.  
\item For any sensor set $\calS\subseteq \calV$, 
\begin{align*}
&\sum_{t=1}^{T}\text{tr}[\Theta_t\Sigma\att{t}{t}(\calS)]=\\
&\sum_{t=1}^{T}\mathbb{E}\left\{\text{tr}[(x_t-\hat{x}_{t,\calS})\tran\Theta_t(x_t-\hat{x}_{t,\calS})]\right\},
\end{align*}
i.e., each $\text{tr}[\Theta_t\Sigma\att{t}{t}(\calS)]$ captures the mean square error that disturbs the control policy $u_{t,\calS}=K_t\hat{x}_{t,\calS}$ away from the perfect state information control policy~$K_tx_t$.
\end{itemize}
Overall, Algorithm~\ref{alg:greedy} selects greedily a sensor set $\algS$,  among all sensor sets $\calS\subseteq \calV$, to bring the imperfect state information control policies $u_{1,\calS}, u_{2,\calS}, \ldots, u_{T,\calS}$ as close as possible to the perfect state information optimal control policies $K_1x_1, K_2x_2, \ldots, K_Tx_T$, and as a result, to achieve the minimum value for Problem~\ref{prob:LQG}.

The reason Algorithm~\ref{alg:greedy} constructs a solution $(\algS, u_{1,\algS}, u_{2,\algS},$ $\ldots, u_{T,\algS})$ for Problem~\ref{prob:LQG} in two separate steps, where the first step regards the controller design ---lines 1--5,--- and the second step regards the sensor selection ---lines 6--23,--- is the following separation property between the controller design and the sensor selection described in Remark~\ref{rem:separation}.

\begin{myremark}[Separation property]\label{rem:separation}
In this paper, we prove that a separation property between the controller design and the sensor selection holds for the sensing-constrained LQG control Problem~\ref{prob:LQG}.  In particular, per Theorem~\ref{th:approx_bound}'s notation, we prove that Problem~\ref{prob:LQG} is equivalent to
\begin{align*}
&\hspace{-1.1em}\min_{\scriptsize \begin{array}{c}
\calS \subseteq \calV, |\calS|\leq k,\\
u_{t,\calS}\in \mathbb{R}^{m_t}
\end{array}} \sum_{t=1}^{T}\mathbb{E}(x\at{t+1}\tran Q_t x\at{t+1}+u_{t,\calS}\tran R_t u_{t,\calS})=\\
&\min_{\calS \subseteq \calV, |\calS|\leq k} \sum_{t=1}^{T}\mathbb{E}(x\at{t+1}\tran Q_t x\at{t+1}+\hat{x}_{t,\calS}\tran K_t\tran R_tK_t \hat{x}_{t,\calS}),
\end{align*}
i.e., the optimal controllers for Problem~\ref{prob:LQG} are decided independently of the optimal sensor set, since the matrices $K_1, K_2$, $\ldots, K_T$ are independent of the selected sensor set, and in particular, are computed as in Algorithm~\ref{alg:greedy}'s lines 1--5.\hfill $\blacktriangle$
\end{myremark}

%Algorithm~\ref{alg:greedy}'s performance is quantified in the following Theorem~\ref{th:approx_bound}, whose proof can be found in the appendix.

\begin{mytheorem}[Performance of Algorithm~\ref{alg:greedy}]\label{th:approx_bound} 
Let
\begin{itemize}
\item for any sensor set $\calS\subseteq\calV$, and control policies $u_1 \in \mathbb{R}^{m_1}, u_2 \in \mathbb{R}^{m_2}, \ldots, u_T \in \mathbb{R}^{m_T}$, $J(\calS, u_1,u_2,\ldots,u_T)$ to be Problem~\ref{prob:LQG}'s cost function, i.e.,
\begin{equation*}
J(\calS, u_1,u_2,\ldots,u_T)=\sum_{t=1}^{T}\mathbb{E}(x\at{t+1}\tran Q_t x\at{t+1}+u_t\tran R_t u_t);
\end{equation*}

\item $g:2^\calV\mapsto \mathbb{R}$ to be such that for any sensor set $\calS \subseteq \calV$, $g(\calS)$ is the value to the cost function $J(\calS, u_{1,\calS},u_{2,\calS},\ldots$, $u_{T,\calS})$ given $\calS$, i.e, 
\begin{equation*}
\hspace{-0.6em}g(\calS)=\min_{\scriptsize \begin{array}{c}
u_{t,\calS} \in \mathbb{R}^{m_t}
\end{array}} J(\calS, u_{1,\calS},u_{2,\calS},\ldots,u_{T,\calS});
\end{equation*}

\item $g^\star$ to be the value of Problem~\ref{prob:LQG}, i.e, 
\begin{equation*}
\hspace{-0.6em}g^\star=\min_{\scriptsize \begin{array}{c}
\calS \subseteq \calV, |\calS|\leq k,\\
u_{t,\calS} \in \mathbb{R}^{m_t}
\end{array}} J(\calS, u_{1,\calS},u_{2,\calS},\ldots,u_{T,\calS}).
\end{equation*}
\end{itemize} 

The following two hold on Algorithm~\ref{alg:greedy}'s performance:
\begin{enumerate}
\item \textit{(Approximation quality)}  Algorithm~\ref{alg:greedy} returns a sensor set $\algS\subseteq \calV$, and gain matrices $K_1, K_2, \ldots,K_T$, such that
\begin{itemize}
\item $|\algS|\leq k$;
\item for control policies $(u_{1,\algS},u_{2,\algS},\ldots,u_{T,\algS})=(K_1\hat{x}_{1,\algS}$, $K_2\hat{x}_{2,\algS},\ldots,K_T\hat{x}_{T,\algS})
$, 
\end{itemize}
\begin{equation}\label{ineq:approx_bound}
\frac{J(\algS, p_{\algS})-g^\star}{g(\emptyset)-g^\star}\leq \min\left[\exp(-\gamma_g), \frac{1-\gamma_g^{k-2}}{1-\gamma_g^{k-1}}\right],
\end{equation}
where $p_{\algS}=(u_{1,\algS},u_{2,\algS},\ldots,u_{T,\algS})$.

\item \textit{(Running time)} Algorithm~\ref{alg:greedy} runs in $O(k|\calV|Tn^{2.4})$ time.

\hfill $\blacktriangle$
\end{enumerate}
\end{mytheorem}

Theorem~\ref{th:approx_bound} implies for Algorithm~\ref{alg:greedy}'s performance:

\textit{a)} Algorithm~\ref{alg:greedy} is the first scalable algorithm for the sensing-constrained LQG control Problem~\ref{prob:LQG}.  In particular, Algorithm~\ref{alg:greedy}'s running time $O(k|\calV|Tn^{2.4})$ is linear both in the number of available sensors $|\calV|$, and the sensor set cardinality constraint $k$, as well as, linear in the Kalman filter's running time across the time horizon $\until{T}$.  Specifically, the contribution $n^{2.4}T$ in Algorithm~\ref{alg:greedy}'s running time comes from the computational complexity of using the Kalman filter to compute the state estimation error covariances $\Sigma\att{t}{t}$ for each $t \in \until{T}$~\cite[Appendix~E]{bertsekas2005dynamic}.

\textit{b)} Algorithm~\ref{alg:greedy}'s achieves an approximate value for the sensing-constrained LQG control Problem~\ref{prob:LQG} that is finitely close to the optimal when the submodularity ratio $\gamma_g$ is non-zero, per Theorem~\ref{th:approx_bound}'s approximation performance bound in ineq.~\eqref{ineq:approx_bound}.  In~particular, the bound in ineq.~\eqref{ineq:approx_bound} improves as the supermodularity ratio $\gamma_g$ increases from $0$ to $1$:
\begin{itemize}
\item for $\gamma_g=0$, the approximation performance bound in ineq.~\eqref{ineq:approx_bound} is uninformative since it is equal to $1$, in which case we get the relation $J(\algS, p_{\algS})-g^\star \leq g(\emptyset)-g^\star$, which always holds since the $J(\algS, p_{\algS}) \leq g(\emptyset)$ holds; specifically, the $J(\algS, p_{\algS}) \leq g(\emptyset)$ holds since the definitions of the set functions $J$ and $g$ in Theorem~\ref{th:approx_bound}, and our proof of separation theorem for Problem~\ref{prob:LQG}, imply $J(\algS, p_{\algS})=g(\algS)$, i.e., $J(\algS, p_{\algS})$ is the value of the cost function in Problem~\ref{prob:LQG} when the sensor set $\algS$ is active, whereas $g(\emptyset)$ is the value of the cost function in Problem~\ref{prob:LQG} when no sensors are active, i.e., $J(\algS, p_{\algS}) \leq g(\emptyset)$. 
\item For $\gamma_g=1$, the approximation performance bound in ineq.~\eqref{ineq:approx_bound} implies an approximate value $63\%$ close to the optimal, since for $\gamma_g=1$, the approximation performance bound in ineq.~\eqref{ineq:approx_bound} is $e^{-1}\simeq .37$.
\end{itemize}
Overall, for non-zero supermodularity ratio $\gamma_g$, ineq.~\eqref{ineq:approx_bound} implies Algorithm~\ref{alg:greedy}'s near-optimal approximation performance.

%\begin{myremark}
%Several supermodularity ratio definitions have been introduced in the literature of set function optimization~\cite{das2011submodular,wang2016approximation,chamon2016near}, and all serve to quantify the approximation performance of the greedy algorithm in solving the cardinality constraint optimization problem $\min_{\calS \subseteq \calV, |\calS|\leq k}f$, where $f:2^\calV\mapsto\mathbb{R}$ is any monotone set function.  The most relevant supermodularity ratio definitions to ours ---Definition~\ref{def:super_ratio}--- are the supermodularity ratio definitions in~\cite{wang2016approximation,chamon2016near}.  In~particular, given  a monotone, non-supermodular set function $f:2^\calV\mapsto\mathbb{R}$, in~\cite{wang2016approximation} the notion of elemental curvature $\alpha_f$ is introduced, which is equal to the reciprocal of $\gamma_f$; and in~\cite{chamon2016near}, a notion of supermodular ratio $r_f$ is introduced, which is equal to $\gamma_f^{k_f}$, where $k_f$ is such that $k_f=O(|\calV|)$; that is,  given  a monotone, non-supermodular set function $f:2^\calV\mapsto\mathbb{R}$, $r_f$ is in general smaller that $\gamma_f$, since for a non-supermodular set function $f$, $\gamma_f<1$. 
%Therefore, the use of the supermodularity ratio Definition~\ref{def:super_ratio} results to the tighter approximation performance bound in Theorem~\ref{th:approx_bound}.
%\hfill $\blacktriangle$
%\end{myremark}

\begin{mytheorem}[Non-zero supermodularity ratio $\gamma_g$]\label{th:submod_ratio}
Let
\begin{itemize}
\item $g:2^\calV\mapsto \mathbb{R}$ to be such that for any sensor set $\calS \subseteq \calV$,
\begin{equation*}
g(\calS)=\min_{\scriptsize \begin{array}{c}
u_{t,\calS} \in \mathbb{R}^{m_t}
\end{array}} \sum_{t=1}^{T}\mathbb{E}(x\at{t+1}\tran Q_t x\at{t+1}+u_{t,\calS}\tran R_t u_{t,\calS});
\end{equation*}
%\item $N_1\in \mathbb{R}^{n_1 \times n_1}$ to solve the system of matrix equations in lines~1 to~5 of Algorithm~\ref{alg:greedy};
\item for any time $t\in \until{T}$, $\Theta_t \in \mathbb{R}^{n_t \times n_t}$ to solve the system of matrix equations in lines~1 to~5 of Algorithm~\ref{alg:greedy};
%\item for any time $t\in \until{T}$, and any sensor set $\calS\subseteq \calV$, $\Sigma\att{t}{t}(\calS)\in \mathbb{R}^{n_t\times n_t}$ to solve the system of matrix equations
%\begin{align*}
%\Sigma\att{t}{t}(\calS)&\leftarrow[\Sigma\att{t}{t-1}(\calS)\inv + C_t(\calS)\tran V_t(\calS)\inv C_t(\calS)]\inv,\\
%\Sigma\att{t}{t-1}(\calS)&\leftarrow A_{t-1} \Sigma\att{t-1}{t-1}(\calS) A_{t-1}\tran + W_{t-1},
%\end{align*} 
%with initial condition the $\Sigma\att{1}{0}(\calS)\leftarrow \Sigma\att{1}{0}$;
%, where $\Sigma\att{1}{0}$ is the covariance of the system's initial condition $x_1$;
\item for any sensor $i \in \calV$, and any time $t \in \until{T}$, $\bar{C}_{i,t}$ to be the noise-weighted measurement matrix $V_{i,t}^{-1/2}{C}_{i,t}$.
\end{itemize}

Consider 
\begin{itemize}
%\item for any time $t\in \{1,2,\ldots, T\}$, $A_t$ to be invertible;
\item the matrix $\sum_{t=1}^{T}\Theta_t$ to be positive definite: $\sum_{t=1}^{T}\Theta_t\succ 0$.
\end{itemize}  
The supermodularity ratio $\gamma_g$ is non-zero.  In particular, for zero process noise ---, for any time $t\in \until{T}$, $w_t=0$,--- and for any time $t\in \until{T}$, $A_t$ invertible, $\gamma_g$'s lower bound simplifies to\footnote{For non-zero process noise, the submodularity ratio $\gamma_g$'s lower bound is found in the proof of Theorem~\ref{th:submod_ratio}.}
\begin{align}\label{ineq:sub_ratio_bound}
\begin{split}
\gamma_g\geq &\frac{\lambda_\min(\sum_{t=1}^T \Theta_t) }{\lambda_\max(\sum_{t=1}^T \Theta_t)}\frac{ \min_{t\in\{1,2,\ldots,T\}}\lambda_\min^2[\Sigma\att{t}{t}(\calV)] }{\max_{t\in\{1,2,\ldots,T\}}\lambda_\max^2[\Sigma\att{t}{t}(\emptyset)]}\\
&\dfrac{1+\min_{i\in\calV, t\in\until{T}}\lambda_\min[\bar{C}_{i} \Sigma\att{t}{t}(\calV) \bar{C}_{i}\tran]}{
 1+\max_{i\in \calV, t\in\until{T}}\lambda_\max[\bar{C}_{i} \Sigma\att{t}{t}(\emptyset) \bar{C}_{i}\tran]}.
 \end{split}
\end{align}

\vspace{-3mm}
\hfill $\blacktriangle$
\end{mytheorem}

The supermodularity ratio bound in ineq.~\eqref{ineq:sub_ratio_bound} improves as: 

\textit{a)} $\lambda_\min(\sum_{t=1}^T \Theta_t) /\lambda_\max(\sum_{t=1}^T \Theta_t)$ increases to $1$, that is, as all eigenvalues of the matrix $\sum_{t=1}^T \Theta_t$ become equal to each other, which implies that the supermodularity ratio bound in ineq.~\eqref{ineq:sub_ratio_bound} improves as on average, across all times $t\in \{1,2,\ldots,T\}$, all the directions $x_t^{(i)}-\hat{x}_{t}^{(i)}$ of the Kalman estimation errors $x_t-\hat{x}_{t}=(x_t^{(1)}-\hat{x}_{t}^{(1)},x_t^{(2)}-\hat{x}_{t}^{(2)},\ldots, x_t^{(n_t)}-\hat{x}_{t}^{(n_t)})$ become equally important in selecting the active sensor set, per Algorithm~\ref{alg:greedy}'s lines~11--32.  For~example, when for all times $t \in \until{T}$ we consider $\lambda=\lambda_\max( \Theta_t)=\lambda_\min(\Theta_t)$, then $\sum_{t=1}^T \Theta_t=\lambda I$, and then for any sensor set $\calS \subseteq \calV$, the set function $\sum_{t=1}^{T}\text{tr}[\Theta_t\Sigma\att{t}{t}(\calS)]$ Algorithm~\ref{alg:greedy} minimizes to select the active sensor set becomes
\begin{align*}
\sum_{t=1}^{T}\text{tr}[\Theta_t\Sigma\att{t}{t}(\calS)]&=
%&\mathbb{E}\left\{\sum_{t=1}^{T}\text{tr}[(x_t-\hat{x}_{t,\calS})\tran\Theta_t(x_t-\hat{x}_{t,\calS})]\right\}=\\
\lambda\sum_{t=1}^{T}\mathbb{E}\left\{\text{tr}(\|	x_t-\hat{x}_{t,\calS}\|_2^2)\right\}\\
&=\lambda\sum_{t=1}^{T}\sum_{i=1}^{n_t}\mathbb{E}\left\{\text{tr}(\|	x_t^{(i)}-\hat{x}_{t,\calS}^{(i)}\|_2^2)\right\};
\end{align*}
i.e., on average, across all times $t\in \{1,2,\ldots,T\}$, all the directions $x_t^{(i)}-\hat{x}_{t}^{(i)}$ of the Kalman estimation errors $x_t-\hat{x}_{t,\calS}$ become equally important in selecting the active sensor set, per Algorithm~\ref{alg:greedy}'s lines~11--32.
Overall, the ratio bound in ineq.~\eqref{ineq:sub_ratio_bound} suggests that it is harder for Algorithm~\ref{alg:greedy} to approximate a solution to Problem~\ref{alg:greedy} as Algorithm~\ref{alg:greedy} needs to differentiate among the directions of the Kalman estimation errors.

\textit{b)} the worst, among all times $t\in \until{T}$, signal to measurement noise fractions that correspond to the last two terms in ineq.~\eqref{ineq:sub_ratio_bound} decrease.  In particular, the last two terms in ineq.~\eqref{ineq:sub_ratio_bound} compare (b.i)~the worst case Kalman estimation quality when all available sensors in $\calV$ are used, which is captured via the two terms of the form $\lambda_\min[\Sigma\att{t}{t}(\calV)]$ and $\lambda_\min[\bar{C}_{i,t} \Sigma\att{t}{t}(\calV) \bar{C}_{i,t}\tran]$, with (b.ii)~the worst case Kalman estimation quality when no sensors are used, which is captured via the two terms of the form $\lambda_\max[\Sigma\att{t}{t}(\emptyset)]$ and $\lambda_\max[\bar{C}_{i,t} \Sigma\att{t}{t}(\emptyset) \bar{C}_{i,t}\tran]$.  Overall, the supermodularity ratio bound in ineq.~\eqref{ineq:sub_ratio_bound} suggests that it is harder for Algorithm~\ref{alg:greedy} to approximate a solution to Problem~\ref{alg:greedy} as the set of available sensors in $\calV$ is inefficient in achieving low estimation error.
%\begin{equation*}
%\begin{array}{l}
%\dfrac{ \min_{t\in\{1,2,\ldots,T\}}\lambda_\min^2[\Sigma\att{t}{t}(\calV)] }{\max_{t\in\{1,2,\ldots,T\}}\lambda_\max^2[\Sigma\att{t}{t}(\emptyset)]};\\
%\dfrac{1+\min_{i\in\calV, t\in\until{T}}\lambda_\min[\bar{C}_{i,t} \Sigma\att{t}{t}(\calV) \bar{C}_{i,t}\tran]}{
% 1+\max_{i\in \calV, t\in\until{T}}\lambda_\max[\bar{C}_{i,t} \Sigma\att{t}{t}(\emptyset) \bar{C}_{i,t}\tran]},
%\end{array}
%\end{equation*}

We capture the frequency Theorem~\ref{th:submod_ratio}'s sufficient condition $\sum_{t=1}^{T} \Theta_t\succ 0$ for non-zero ratio $\gamma_g$  with Theorem~\ref{th:freq}.

\begin{mytheorem}\label{th:freq}
%Let  $N_1\in \mathbb{R}^{n_1 \times n_1}$ to solve the system of matrix equations in lines~1 to~5 of Algorithm~\ref{alg:greedy}, and 
Consider the noiseless perfect state information LQG problem where for any time $t\in \{1,2,\ldots, $ $ T\}$, the state $x_t$ is known to each controller $u_t$, ---$u_t=u_t(x_t)$,--- and the process noise $w_t$ is zero, i.e., the optimization problem
\begin{equation}\label{pr:perfect_state}
\min_{u_t\in \mathbb{R}^{m_t}}\sum_{t=1}^{T}\left.[x\at{t+1}\tran Q_t x\at{t+1}+u_{t}(x_t)\tran R_t u_{t}(x_t)]\right|_{w_t=0}.
\end{equation}

Let for any time $t\in \{1,2,\ldots, T\}$, $A_t$ to be invertible; the strict inequality $\sum_{t=1}^{T} \Theta_t\succ 0$ holds if and only if for all non-zero initial conditions~$x_1\in\mathbb{R}^{n_1}$,
%for any non-zero initial condition $x_1\in\mathbb{R}^{n_1}$, the all-zero control policy $(u_1,u_2,\ldots,$ $u_T)=(0,0,\ldots, 0)$ is suboptimal for the noiseless perfect state-information LQG problem in eq.~\eqref{pr:perfect_state}, i.e.,
\begin{align*}
&(u_1,u_2,\ldots,u_T)=(0,0,\ldots, 0)\notin \\
&\arg\min_{u_t\in \mathbb{R}^{m_t}}\sum_{t=1}^{T}\left.[x\at{t+1}\tran Q_t x\at{t+1}+u_{t}(x_t)\tran R_t u_{t}(x_t)]\right|_{w_t=0}.
\end{align*}

\vspace{-3mm}
\hfill $\blacktriangle$
\end{mytheorem}

Theorem~\ref{th:freq} suggests that if for any non-zero initial condition~$x_1$ the all-zeroes control policy $(u_1,u_2,\ldots,u_T)=(0,$ $0,$ $\ldots, 0)$ is suboptimal for the noiseless perfect state information LQG problem in eq.~\eqref{pr:perfect_state}, then Theorem~\ref{th:submod_ratio}'s sufficient condition $\sum_{t=1}^{T} \Theta_t\succ 0$ for non-zero supermodularity ratio $\gamma_g$ holds.  The all-zeroes control policy is always suboptimal for the noiseless perfect state information LQG problem in eq.~\eqref{pr:perfect_state} for appropriate LQG cost matrices $Q_1, Q_2,$ $\ldots,$ $Q_T$ and $R_1, R_2, \ldots, R_T$, as implied by Proposition~\ref{prop:iff_for_all_zero_control} below.
% We illustrate the intuition behind Theorem~\ref{th:freq} starting with an example:  Consider a system of the form $x_{t+1}=x_t$, that is, for any $t\in\until{T}$, $x_t=x_1$.  Then, the matrix $\Xi=[K_1\tran, K_2\tran, \ldots, K_T\tran]\tran$ has rank $n$, since the optimal control policies for the noiseless perfect state information LQG problem in eq.~\eqref{pr:perfect_state} have the form $K_tx_t=K_tx_1$, and for all non-zero $x_1$, $(u_1\tran,u_2\tran,\ldots,u_T\tran)\tran=\Xi x_1 \neq 0$.  At the same time,  $\sum_{t=1}^{T}\Theta_t=\Xi\tran  \text{diag}(M_1, M_2, \ldots, M_T) \Xi$, and as a result, for all non-zero $x_1$, $\sum_{t=1}^{T}\Theta_tx_1\neq 0$, since $\Xi x_1\neq 0$, and $\text{diag}(M_1, M_2, \ldots, M_T)$ is invertible.  Overall, .  A class of systems where is the fully unstable systems, where all eigenvalues of the system matrices $A_t$ are strictly positive, since for unstable system the optimal control policies are necessarily non-zero to make the closed-loop system stable.

\begin{myproposition}\label{prop:iff_for_all_zero_control}
Let $N_1\in \mathbb{R}^{n_1 \times n_1}$ to solve the system of matrix equations in lines~1--5 of Algorithm~\ref{alg:greedy}.  For all non-zero initial conditions~$x_1\in\mathbb{R}^{n_1}$, the control policy $(u_1,u_2,$ $\ldots,$ $u_T)=(0,0,\ldots, 0)$ is suboptimal for the noiseless perfect state information LQG problem in eq.~\eqref{pr:perfect_state}
if and only if 

\beq\label{ineq:iff_for_all_zero_control}
\sum_{t=1}^{T} A_1\tran \cdots A_t\tran Q_t A_t\cdots A_1\succ N_1.
\eeq

\vspace{-3mm}
\hfill $\blacktriangle$
\end{myproposition}

The strict ineq.~\eqref{ineq:iff_for_all_zero_control} holds for appropriate LQG cost matrices $Q_1, Q_2,$ $\ldots,$ $Q_T$ and $R_1, R_2, \ldots, R_T$, as, for example, when the control cost matrices $R_1, R_2, \ldots, R_T$ are closer to zero than the state cost matrices $Q_1, Q_2,$ $\ldots,$ $Q_T$, that is, as when the LQG cost function penalizes the state vector values more than the control vector values.  For example, consider the case where the LQG cost matrix $R_1$ tends to zero, i.e., consider $\epsilon$ such that $R_1\preceq \epsilon I$, and $\epsilon\longrightarrow 0$; then, for any~$Q_1$, and for $A_1$ invertible per conditions of Theorem~\ref{th:freq}, the strict ineq.~\eqref{ineq:iff_for_all_zero_control} holds for $\epsilon$ small, since $N_1\preceq \epsilon A_1\tran (\epsilon S_1\inv +B_1 B_1\tran)\inv A_1\longrightarrow 0$ for $\epsilon \longrightarrow0$.  In particular, $R_1\preceq \epsilon I$, and~\cite[Proposition~8.5.5]{bernstein2005matrix},\footnote{\cite[Proposition~8.5.5]{bernstein2005matrix} states that for any positive definite matrices $M_1$ and $M_2$ such that $M_1\preceq M_2$, $M_2\inv\preceq M_1\inv$.} imply $R_1\inv \succeq I/\epsilon$, and as a result, $S_1\inv+ B_1 R_1\inv B_1\tran\succeq (\epsilon S_1\inv+ B_1 B_1\tran)/\epsilon$, which in turn implies $(S_1\inv+ B_1 R_1\inv B_1\tran)\inv\preceq \epsilon(\epsilon S_1\inv+ B_1 B_1\tran)\inv$, and consequently, $N_1\preceq \epsilon A_1\tran (\epsilon S_1\inv +B_1 B_1\tran)\inv A_1$.

Overall, Algorithm~\ref{alg:greedy} is the first scalable algorithm for the sensing-constrained LQG control Problem~\ref{prob:LQG}, and for appropriate LQG cost matrices $Q_1, Q_2, \ldots, Q_T$ and $R_1, R_2, \ldots, R_T$, Algorithm~\ref{alg:greedy} achieves near-optimal approximate performance.

==> tex/algorithm3.tex <==
%!TEX root = ../main.tex

\begin{algorithm}[t]
\caption{Optimal control policy design for Problem~\ref{prob:LQG}.}
\begin{algorithmic}[1]
\REQUIRE Time horizon $T$, and for all $t=1,2,\ldots, T$, system matrix~$A_t$, input matrix $B_t$, and cost matrices $Q_t$ and $R_t$.
\ENSURE Matrices $K_1, K_2$, $\ldots, K_T$ and $\Theta_1, \Theta_2$, $\ldots, \Theta_T$.
\STATE $N_{T+1}\leftarrow 0_{n_{T}\times n_T}$; $t\leftarrow T$;
\WHILE {$t\geq 1$} 
\STATE{$S_t \leftarrow Q_t + N_{t+1}$;}
\STATE{$N_t \leftarrow A_t\tran (S_t\inv+B_tR_t\inv B_t\tran)\inv A_t$;}
\STATE{$M_t \leftarrow B_t\tran S_t B_t + R_t$;}
\STATE{$K_t \leftarrow - M_t\inv B_t\tran S_t A_t$;}
\STATE{$\Theta_t\leftarrow K_t\tran M_t K_t$;}
\STATE{$t\leftarrow t-1$;}
\ENDWHILE
\end{algorithmic} \label{alg:control}
\end{algorithm}

==> tex/figure_formation_costVShorizon.tex <==
%!TEX root = ../main.tex

\renewcommand{\mpw}{4.5cm}
\begin{figure}[t]
\hspace{-4mm}
\begin{minipage}{\textwidth}
\begin{tabular}{cc}%
\begin{minipage}{\mpw}%
\centering
\includegraphics[width=1.05\columnwidth]{results-formationControl-costOverHorizon/figure-formationControl-singleRun-T20-maxT20-maxT20-het0-mpc0-n4-k6} \\
(a) homogeneous 
\end{minipage}
& 
\begin{minipage}{\mpw}%
\centering%
\includegraphics[width=1.05\columnwidth]{results-formationControl-costOverHorizon/figure-formationControl-singleRun-T20-maxT20-maxT20-het1-mpc0-n4-k6} \\
(b) heterogeneous 
\end{minipage}
\end{tabular}
\end{minipage}%
\vspace{-1mm}
\caption{\label{fig:snapshots}
Snapshots of the feature selection performed by the different techniques  during a sharp
}\vspace{-5mm}
\end{figure}
